Efficiently Finding Higher-Order Mutants

Higher-order mutation has the potential for improving major drawbacks of traditional first-order mutation, such as by simulating more realistic faults or improving test optimization techniques. Despite interest in studying promising higher-order mutants, such mutants are difficult to find due to the exponential search space of mutation combinations. State-of-the-art approaches rely on genetic search, which is often incomplete and expensive due to its stochastic nature. First, we propose a novel way of finding a complete set of higher-order mutants by using variational execution, a technique that can, in many cases, explore large search spaces completely and often efficiently. Second, we use the identified complete set of higher-order mutants to study their characteristics. Finally, we use the identified characteristics to design and evaluate a new search strategy, independent of variational execution, that is highly effective at finding higher-order mutants even in large code bases.

==> resources/itemset.tex <==
ROR&==&<&23\%&8\%&46\%&39\%&29\%\\
ROR&==&>&24\%&6\%&32\%&21\%&21\%\\
ROR&==&!=&20\%&5\%&9\%&35\%&17\%\\
AOR&+&\%&15\%&10\%&9\%&36\%&17\%\\
ROR&==&<=&25\%&4\%&38\%&0\%&17\%\\
AOR&+&/&13\%&19\%&9\%&21\%&15\%\\
AOR&+&*&23\%&7\%&16\%&14\%&15\%\\
AOR&+&-&18\%&19\%&8\%&14\%&15\%\\
ROR&==&>=&22\%&15\%&15\%&0\%&13\%\\
LCR&\&\&&||&24\%&16\%&9\%&1\%&12\%\\


==> sections/__latexindent_temp.tex <==
    \end{tabular}

==> sections/serena.tex <==
% \newpage

% \todo{serena's paper}

% Mutation testing is an effective but time consuming method for gauging the quality of a test suite. It functions by repeatedly making changes, called mutants, to the source code and checking whether the test suite fails (i.e., whether the mutant is \textit{killed})~\cite{demillo}. Recent work~\cite{jiaHigher09} has shown cases in which applying multiple changes, called a \textit{higher order mutation}, is more difficult to kill than a single change, called a \textit{first order mutation}. Specifically, a special kind of higher order mutation, called a \textit{strongly subsuming higher order mutation (SSHOM)}, can enable equivalent accuracy in assessing the quality of the test suite with fewer executions of tests. Little is known about these \sshoms{}, as they are difficult to find. Jia et. al~\cite{jiaHigher09} used a genetic search to find \sshoms; however, since it runs over many generations and has an element of randomness, the algorithm is time consuming and the results are often incomplete.

% Our goal in this research is to identify a faster, more reliable method for finding \sshoms{} in order to characterize them in the future. We propose an approach based on variational execution to find \sshoms. Preliminary results indicate that variational execution performs better than the existing genetic algorithm in terms of speed and completeness of results. Out of a set of 33 first order mutations, our variational execution approach finds all 38 \sshoms{} in 4.5 seconds, whereas the genetic algorithm only finds 36 of the 38 \sshoms{} in 50 seconds.

% \section{Approach}

% % \begin{itemize}
% %     \item bg on varex and why we use it
% %     \item How we use it for mutation testing
% %     \begin{itemize}
% %         \item encode mutants as conditionals
% %         \item formula with 3 specifications
% %     \end{itemize}
% % \end{itemize}

% In this section, we discuss our approach to finding \sshoms{} using variational execution.

% \subsection{Variational Execution}

% Variational execution is a dynamic analysis that explores the behavior of a program under all inputs by sharing redundant executions. It was originally designed to examine the interactions of configuration options in a program~\cite{MWK+:ASE16}. The output of variational execution is an expression for the input conditions for which certain outputs are achieved.
% %It represents runtime values as \textit{conditional values} and uses \textit{variability contexts} to represent the conditions in which an instruction is executed~\cite{MWK+:ASE16}.

% We encode all possible first order mutants as runtime variables. An example is shown in Listing~\ref{lst:mut}. Then, we can use variational execution to efficiently and exhaustively explore the behavior of the test suite under all combinations of mutants. Variational execution will then output the mutant configurations in which a test case fails as a \textit{variability context}, or a propositional formula over the input options. For example, let's say we have two tests for the code example in Listing~\ref{lst:mut}:

% \begin{enumerate}
% 	\item \texttt{assertTrue(equalsThree(1, 2));}
% 	\item \texttt{assertFalse(equalsThree(3, 4));}
% \end{enumerate}

% \noindent{}Variational execution would output two variability contexts:

% \begin{enumerate}
% 	\item \texttt{\{test1 failed\} : (m0 $\wedge \neg$m1) $\vee$ ($\neg$m0 $\wedge$ m1)}
% 	\item \texttt{\{test2 failed\} : m1}
% \end{enumerate}

% \noindent{}From these variability contexts, we derive \sshoms{} using logical reasoning, which we will discuss next.


% \begin{lstlisting}[language=diff, basicstyle=\ttfamily, caption=Diff of mutations encoded as runtime variability., captionpos=b, frame=tb, float=tp, numbers=left, label=lst:mut, tabsize=2, escapechar=~]
% boolean equalsThree(int a, int b) {
% -  int c = a + b;
% +  int c = m0 ? a - b : a + b;
% -  return c == 3;
% +  return m1 ? c != 3 : c == 3;
% }
% \end{lstlisting}
% %boolean eqThree(int a, int b) {
% %  int c = m0 ? a - b : a + b;
% %  return m1 ? c != 3 : c == 3;
% %}


% \subsection{Finding Strongly Subsuming Higher Order Mutants}

% Current approaches to finding \sshoms{}, such as genetic algorithms or greedy algorithms, are search based~\cite{jiaHigher09}. In contrast, our approach directly generates \sshoms{}. This approach uses the output of variational execution to construct a formula that encodes the definition of a \sshom{} and evaluates to true for all \sshoms{}. Since this formula is a satisfiability problem, we can use a BDD or SAT solver to cheaply find \sshoms{}.

% To derive the formula, we outline the criteria for identifying \sshoms{} as defined by Jia et. al~\cite{jiaHigher09} and construct a logical expression for each criterion.

% Let $T$ be the set of all tests, $M$ be the set of all first order mutants, and $f(t)$ be the propositional formula for the mutant configurations in which test $t$ fails, as demonstrated in the variability contexts in the previous section. Let $\Gamma(m,t)$ be the result of evaluating $f(t)$ with first order mutant $m$; in other words, whether or not test $t$ fails with first order mutant $m$. The criteria for \sshoms{} follow:

% \begin{enumerate}
% 	\item The \sshom{} must fail at least one test (must not be an equivalent mutant)
% \end{enumerate}
% \begin{equation}
% \label{not-eq}
% \bigvee\limits_{t \in T} f(t)
% \end{equation}

% \noindent{}In order to find the mutant configurations in which at least one test fails, it is sufficient to take the disjunction of the conditions in which each test fails. Thus, if a mutant configuration successfully kills a test, the whole expression is true.

% \begin{enumerate}
% 	\setcounter{enumi}{1}
% 	\item Every test that fails the \sshom{} must fail each constituent first order mutant
% \end{enumerate}
% \begin{equation}
% \label{homsubset}
% \bigwedge\limits_{t \in T} (f(t) \Rightarrow \bigwedge\limits_{m \in M} {\underbrace{\vrule width0pt depth4pt ( \neg m \vee \Gamma(m, t) )}_{\strut\mathclap{ \text{Either } m \text{ is not included or is killed by }t}}})
% \end{equation}

% \noindent{}A certain mutant configuration (i.e. higher order mutant) killing a test implies one of two things for each first order mutant in the program: either the first order mutant is not in the higher order mutant ($\neg m$) or the test fails for the first order mutant ($\Gamma(m,t)$). This must hold over all tests and first order mutants.

% In addition, we can optimize for \sshoms{} that are harder to kill than the constituent first order mutants, excluding those that are equally difficult to kill~\cite{jiaHigher09}. We call these \textit{strictly subsuming higher order mutants} and add a third criteria to find them.

% \begin{enumerate}
% 	\setcounter{enumi}{2}
% 	\item The set of tests that kill the higher order mutant must be a strict subset of the tests that kill all the first order mutants
% \end{enumerate}
% \begin{equation}
% \label{strict-formula}
% \bigvee\limits_{t \in T} \big(\overbrace{\strut\neg f(t)}^{\mathclap{\strut\text{The selected mutants do not kill the test}}} \wedge \bigwedge\limits_{m \in M} {\underbrace{\vrule width0pt depth4pt ( \neg m \vee \Gamma(m, t) )}_{\strut\mathclap{ \text{Either } m \text{ is not included or is killed by }t}}}\big)
% \end{equation}

% \noindent{}If we replace all the constituent first order mutants with this strictly subsuming higher order mutant, then we will have a smaller set of tests that can kill the set of mutants. As such, there must exist at least one test that does not fail for the included mutants but does fail for each first order mutant of the higher order mutant.

% To compute the \sshoms, we take the conjunction of Equations~\ref{not-eq}~and~\ref{homsubset} (and Equation~\ref{strict-formula} for strictly subsuming higher order mutants) and use a BDD or SAT solver to iteratively get all satisfiable solutions. Thus, this formula is guaranteed to generate all of the possible \sshoms{} for the given set of first order mutants, the given test set.

\section{Preliminary Evaluation}

% \begin{itemize}
%     \item explain setup
%     \begin{itemize}
%         \item reimplementation of ga
%         \item setup of ga
%         \item setup of varex
%         \item specs of machine
%         \item Triangle (and why we use it)
%         \item Monopoly if we get that far
%     \end{itemize}
%     \item graph
%     \begin{itemize}
%         \item short paragraph of explanation
%     \end{itemize}
% \end{itemize}

We compared three approaches to finding \sshoms{}: a naive exhaustive search method, the state of the art genetic algorithm outlined in the work of Jia et. al~\cite{jiaHigher09,harmanAngels14}, and our variational execution approach.

The exhaustive search serves as a baseline. We iterate through all pairs of first order mutants, then all triples, and so on. For each candidate higher order mutant, we run the tests and check whether the results indicate that the higher order mutant is strongly subsuming. This algorithm has an exponential runtime.

As we could not find an existing implementation of the genetic algorithm, we reimplemented the algorithm presented by Jia et. al~\cite{jiaHigher09,harmanAngels14} with a few modifications optimizing for the current limited number of mutation operators.

We tested the three approaches on the program \textit{Triangle}. Triangle is a simple program that takes three integers representing three side lengths of a triangle and outputs whether the triangle is equilateral, scalene, isosceles, or invalid. This program is used in mutation testing literature and was used to test the original genetic algorithm for finding \sshoms~\cite{jiaHigher09}. Triangle contains about 40 lines of code and 33 first order mutations. The test suite we used was generated by EvoSuite~\cite{Fraser:2011:EAT:2025113.2025179}, with a few test cases manually added for completeness.

%% pick one of these graphs
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{comparison-graph-linear.pdf}
%     \caption{The number of mutants found over time in Triangle}
%     \label{fig:comp-lin}
% \end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{comparison-graph-log.pdf}
	\caption{The number of mutants found over time in Triangle. Note, the x axis is in log scale.}
	\label{fig:comp-log}
\end{figure}

After running the three algorithms on Triangle, we plotted the number of \sshoms{} found over time, as shown in Figure \ref{fig:comp-log}. Since the variational execution and exhaustive search always find all the \sshoms{}, we establish that from the 33 first order mutations, there are 38 total \sshoms{}. The exhaustive search finds all the \sshoms{} in just under 4 minutes, but does not terminate as it continues testing more higher order mutants. The genetic algorithm finds its last \sshom{} after 50 seconds but it only finds 36 of the 38 \sshoms. Due to the random nature of the genetic algorithm, all four of our trials resulted in the genetic algorithm eventually hanging and no longer able to find more \sshoms. The variational execution approach finds all the \sshoms{} 50 times faster than the exhaustive search and 10 times faster than the genetic algorithm approach. The variational execution approach takes 4 seconds to run variational execution and 0.5 seconds to find all the \sshoms{}, a total of 4.5 seconds. Although variational execution takes a while, finding the \sshoms{} is very quick as satisfiability checks are inexpensive and fast compared to running a test suite, as happens in the exhaustive search and genetic algorithm.

\section{Conclusions}

% \begin{itemize}
%     \item we expect this to scale
%     \item future work
%     \item "this is promising"
% \end{itemize}

We propose a new way of finding \sshoms{} using variational execution and compared it to the state of the art genetic algorithm and a baseline exhaustive search method. The significant improvement in performance in a small program like Triangle leads us to believe that the variational execution approach is promising. In addition to extending to larger programs, future work includes analyzing the \sshoms{} and finding any defining characteristics.


==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.8	//
Abbreviations and Acronyms	conference_041818.tex	/^\\subsection{Abbreviations and Acronyms}\\label{AA}$/;"	b
Acknowledgment	conference_041818.tex	/^\\section*{Acknowledgment}$/;"	s
Approach	sections/approach.tex	/^\\section{Approach}$/;"	s
Approaches to Finding SSHOMs	sections/relatedwork.tex	/^\\paragraph{Approaches to Finding SSHOMs}$/;"	P
Authors and Affiliations	conference_041818.tex	/^\\subsection{Authors and Affiliations}$/;"	b
Baseline Search Strategies	sections/evaluation.tex	/^\\paragraph{Baseline Search Strategies}$/;"	P
Characteristics of SSHOMs	sections/relatedwork.tex	/^\\paragraph{Characteristics of SSHOMs}$/;"	P
Combinatorial Explosion	sections/approach.tex	/^\\paragraph{Combinatorial Explosion} Recent studies show that combinatorial $/;"	P
Conclusions	sections/conclusion.tex	/^\\section{Conclusions}$/;"	s
Conclusions	sections/serena.tex	/^\\section{Conclusions}$/;"	s
Discussions	sections/HOM.tex	/^\\subsection{Discussions}$/;"	b
Ease of Use	conference_041818.tex	/^\\section{Ease of Use}$/;"	s
Encoding SSHOMs Search as a Boolean Satisfiability Problem	sections/approach.tex	/^\\subsection{Encoding SSHOMs Search as a Boolean~Satisfiability Problem}\\label{subsec:sat}$/;"	b
Environment Barrier	sections/approach.tex	/^\\paragraph{Environment Barrier} Variational execution needs to deal with environment barrier carefully when $/;"	P
Equations	conference_041818.tex	/^\\subsection{Equations}$/;"	b
Evaluation	sections/evaluation.tex	/^\\section{Evaluation}\\label{sec:evaluation}$/;"	s
Experimental Setup	sections/evaluation.tex	/^\\subsection{Experimental Setup}$/;"	b
Figures and Tables	conference_041818.tex	/^\\subsection{Figures and Tables}$/;"	b
Finding SSHOMs	sections/HOM.tex	/^\\subsection{Finding SSHOMs}$/;"	b
Higher Order Mutants	sections/HOM.tex	/^\\section{Higher-Order Mutants}$/;"	s
Identify the Headings	conference_041818.tex	/^\\subsection{Identify the Headings}$/;"	b
Introduction	conference_041818.tex	/^\\section{Introduction}$/;"	s
Introduction	sections/introduction.tex	/^\\section{Introduction}$/;"	s
LaTeX Specific Advice	conference_041818.tex	/^\\subsection{\\LaTeX-Specific Advice}$/;"	b
Limitations	sections/approach.tex	/^\\subsection{Limitations}\\label{subsec:limitations}$/;"	b
Maintaining the Integrity of the Specifications	conference_041818.tex	/^\\subsection{Maintaining the Integrity of the Specifications}$/;"	b
Measurements	sections/evaluation.tex	/^\\paragraph{Measurements} All experiments were performed on AWS EC2 instances, each of which has an Intel 4-core Xeon CPU $/;"	P
Mutants Generation	sections/approach.tex	/^\\subsection{Mutants Generation}$/;"	b
Overview	sections/approach.tex	/^\\subsection{Overview}\\label{subsec:overview}$/;"	b
Positioning Figures and Tables	conference_041818.tex	/^\\paragraph{Positioning Figures and Tables} Place figures and tables at the top and $/;"	P
Preliminary Evaluation	sections/serena.tex	/^\\section{Preliminary Evaluation}$/;"	s
Prepare Your Paper Before Styling	conference_041818.tex	/^\\section{Prepare Your Paper Before Styling}$/;"	s
References	conference_041818.tex	/^\\section*{References}$/;"	s
Related Work	sections/relatedwork.tex	/^\\section{Related Work}$/;"	s
Research Questions	sections/evaluation.tex	/^\\subsection{Research Questions}\\label{subsec:rqs}$/;"	b
Results	sections/evaluation.tex	/^\\subsection{Results}$/;"	b
Some Common Mistakes	conference_041818.tex	/^\\subsection{Some Common Mistakes}\\label{SCM}$/;"	b
Strongly Subsuming Higher Order Mutants SSHOMs	sections/HOM.tex	/^\\subsection{Strongly Subsuming Higher-Order Mutants (SSHOMs)}\\label{sec:sshom}$/;"	b
Subject Systems	sections/evaluation.tex	/^\\paragraph{Subject Systems}$/;"	P
Threats to Validity	sections/evaluation.tex	/^\\subsection{Threats to Validity} $/;"	b
Units	conference_041818.tex	/^\\subsection{Units}$/;"	b
Usefulness of Higher Order Mutants	sections/relatedwork.tex	/^\\paragraph{Usefulness of Higher-Order Mutants}$/;"	P
Variational Execution	sections/approach.tex	/^\\subsection{Variational Execution}\\label{subsec:ve}$/;"	b
Variational Execution	sections/relatedwork.tex	/^\\paragraph{Variational Execution}$/;"	P
textbf Discussions	sections/evaluation.tex	/^\\paragraph{\\textbf{Discussions}} From a complete set of SSHOMs, we study their characteristics with $/;"	P
textbf RQ1 Efficiency of finding SSHOMs	sections/evaluation.tex	/^\\paragraph{\\textbf{RQ1: Efficiency of finding SSHOMs}} $/;"	P
textbf RQ2 Test Efficiency	sections/evaluation.tex	/^\\paragraph{\\textbf{RQ2: Test Efficiency}}$/;"	P
textbf RQ3 Locality	sections/evaluation.tex	/^\\paragraph{\\textbf{RQ3: Locality}} To see how constituent first-order mutants $/;"	P
textbf RQ4 Order	sections/evaluation.tex	/^\\paragraph{\\textbf{RQ4: Order}} To inform bounds of future search strategies, we plot the $/;"	P
textbf RQ5 Combination Strategies	sections/evaluation.tex	/^\\paragraph{\\textbf{RQ5: Combination Strategies}} With this RQ we hope to inform future research $/;"	P

